A Harmonic Extension Approach for Collaborative Ranking

We present a new perspective on graph-based methods for collaborative ranking for recommender systems. Unlike user-based or item-based methods that compute a weighted average of ratings given by the nearest neighbors, or low-rank approximation methods using convex optimization and the nuclear norm, we formulate matrix completion as a series of semi-supervised learning problems, and propagate the known ratings to the missing ones on the user-user or item-item graph globally. The semi-supervised learning problems are expressed as Laplace-Beltrami equations on a manifold, or namely, harmonic extension, and can be discretized by a point integral method. We show that our approach does not impose a low-rank Euclidean subspace on the data points, but instead minimizes the dimension of the underlying manifold. Our method, named LDM (low dimensional manifold), turns out to be particularly effective in generating rankings of items, showing decent computational efficiency and robust ranking quality compared to state-of-the-art methods.

==> LDMM0.tex <==
In this section, we give another interpretation of our method based on the low dimensionality of the user manifold. In the user-by-item rating system, a user is 
represented by an $n$-dimensional vector that consists of the ratings to $n$ items. The user manifold is a manifold embedded in $\mathbb{R}^n$.
Usually, $n$, the number of items, is a large number in the order of $10^3\sim 10^6$. The intrinsic dimension of the user manifold is much less than $n$. Based on this observation, 
it is natural to recover the rating matrix by looking for the user manifold with the lowest dimension. This idea implies the following optimization problem.
\begin{align}
  \label{eq:model-manifold}
 & \min_{X\in \mathbb{R}^{m\times n},\atop \M\subset \mathbb{R}^n} \quad\dim(\mathcal{M}),\\
 &\text{subject to:}\quad P_{\Omega}(X)=P_{\Omega}(A)  , \quad \mathcal{U}(X)\subset \M.\nonumber
\end{align}
where $\dim(\M)$ is the dimension of the manifold $\M$, and $\mathcal{U}(X)$ is the user set corresponding to the rows of $X$. 



%Next, we need to give a formula to compute $\dim(\mathcal{M})$ using differential geometry.
Next, we need to give a mathematical expression to compute $\dim(\mathcal{M})$.
Here we assume $\M$ is a smooth manifold embedded in $\mathbb{R}^n$.
Let $\alpha_i, \; i=1,\cdots,d$ be the coordinate functions on $\M$, i.e.
\begin{align}
  \label{eq:fun-coordinate}
  \alpha_i(\bx)=x_i,\quad \forall \bx=(x_1,\cdots,x_n)\in \M
\end{align}
Using differential geometry, we have the following formula \cite{LDMM_image}.
\begin{proposition} 
\label{prop:dim}
Let $\M$ be a smooth submanifold isometrically embedded in $\mathbb{R}^n$. For any $\bx\in \M$,  
  \begin{align*}
    \dim(\M)=\sum_{j=1}^n\|\nabla_\M\alpha_j(\bx)\|^2
  \end{align*}
where $\nabla_\M$ is the gradient in the manifold $\M$.
\end{proposition}


Using the above proposition, the optimization problem \eqref{eq:model-manifold} can be rewritten as
\begin{align}
  \label{eq:model-manifold-grad}
&  \min_{X\in \mathbb{R}^{m\times n},\atop \M\subset \mathbb{R}^d} \quad \sum_{i=1}^d\|\nabla_{\M} f_i\|_{L^2(\M)}^2,\\
& \text{subject to:}\quad
f_i(x_j)|_{U_i}=a_{ij}, \quad \mathcal{U}(X)\subset \M,\nonumber
\end{align}
where
\begin{equation}
  \label{eq:def-l2}
  \|\nabla_{\M} f_i\|_{L^2(\M)}=\left(\int_{\M} \|\nabla_{\M} f_i(\bx)\|^2\mathd {\bx}\right)^{1/2}.
\end{equation}
This is the optimization problem we solved in Section \ref{harmonic} and Section \ref{discretization}.
% \begin{align}
%   \label{eq:model-manifold-noise}
%   \min_{f\in \mathbb{R}^{m\times n}} \quad \sum_{i=1}^d\|\nabla_{\Mp} \alpha_i\|_{L^2(\Mp)}^2+\lambda \|y-\Phi f\|_{l^2}^2.
% \end{align}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper0104"
%%% End:


==> LPIM.tex <==
\begin{figure*}[!t]
\centering
\subfloat [] {\includegraphics[width=0.25\textwidth]{localized}}
\hspace{0.1\textwidth}
\subfloat [] {\includegraphics[width=0.25\textwidth]{localized2}}
\hspace{0.1\textwidth}
\subfloat [] {\includegraphics[width=0.18\textwidth]{localized3}}
\caption{Illustration of the localized scheme in point integral method with $10$ users ($m=10$). (a) The sparse similarity matrix $W$ and the $j$-th column of the incomplete rating matrix $A$ for some item $j$. (b) We identify the set of neighbors $\mathcal{N}(\Omega_j)$ from the rows of $W$ that correspond to $\Omega_j$. In this example, $\mathcal{N}(\Omega_j) = \{5,6,8,9\}$. (c) We extract the submatrix of $W$ with rows and columns in $S_j = \Omega_j \cup \mathcal{N}(\Omega_j)$, and propagate the labels (by solving Eq. (\ref{reducedsystem})) on this subgraph only. Note that in this example, $W_{S_j,S_j}$ does not have full rank, but $L_{S_j,S_j}= D(W_{S_j,S_j}) - W_{S_j,S_j}$ is always non-singular.}
\label{fig:illus_localized}
\end{figure*}

In the previous section, we solved the discretized harmonic extension problem by filling in all the unobserved ratings. However, this is neither efficient nor necessary to generate the top recommended items in a real scenario. We would rather predict only the ratings that are most likely to appear.

The input rating matrix $A$ is often extremely sparse. In order to obtain a scalable algorithm, we have to keep everything sparse in our algorithm. In particular, we cannot afford to generate a dense rating matrix in any intermediate iteration or the final result. (Generating a sparse similarity matrix $W$ from the incomplete rating matrix $R$ will be discussed in the next section.)

Let $\Omega_j=\{i \in \mathbb{Z}|A_{i,j} \text{ is observed}\}$ be the set of indices of users who rated the item $j$. To restrict the set of entries to fill in for the column $R_{:,j}$, our \textbf{assumption} is that the users most likely to rate the item $j$ are those who are {\em similar} to the users in $\Omega_j$. Now we describe a way to define the set of neighbors of each user on a graph (note that there may be other definitions of the neighborhood):
\begin{equation}
\label{neighbors}
\mathcal{N}(i) = \{i' \in \mathbb{Z} | W_{i,i'} \neq 0\},
\end{equation}
and consequently, the set of all the users that are similar to the users in $\Omega_j$ is:
\begin{equation}
\label{neighbors_omega}
\mathcal{N}(\Omega_j) = \bigcup_{i \in \Omega_j} \mathcal{N}(i).
\end{equation}
Then, we extract the subgraph with nodes in the index set
\begin{equation}
\label{subgraph}
S_j=\Omega_j \cup \mathcal{N}(\Omega_j),
\end{equation}
and propagate the known ratings on this subgraph only. Numerically, we solve the linear system for $r \in \mathbb{R}^m$
\begin{equation}
\label{reducedsystem}
L_{S_j,S_j} r_{S_j} + \mu W_{S_j,\Omega_j} r_{\Omega_j} = \mu W_{S_j, \Omega_j} R_{S_j, j},
\end{equation}
which is much smaller than the one defined on the entire user-user graph, and update $R_{S_j, j}$, the predicted ratings for item $j$, with $r_{S_j}$. Thus, we obtain a partial solution of the harmonic extension problem. Our localized scheme is illustrated in Figure \ref{fig:illus_localized}. Our algorithm for harmonic extension with localized point integral method is summarized in Algorithm \ref{alg:localpim}.

\begin{algorithm}[!t]
\caption{Harmonic extension algorithm using localized point integral method}
\label{alg:localpim} \centering
\begin{algorithmic}[1]
\REQUIRE Incomplete rating matrix $A \in \mathbb{R}^{m \times n}$
\STATE $R \leftarrow A$
\REPEAT
\STATE Compute the similarity matrix $W$ based on $R$ (Algorithm \ref{alg:sim_matrix})
\FOR {$i=1$ to $n$}
\STATE Fill random values into $R_{S_j \backslash \Omega_j, j}$
\STATE $r \leftarrow$ Solution of the linear system (\ref{reducedsystem}) with $S_j$ defined in (\ref{subgraph})
\STATE $R_{S_j,j} \leftarrow r_{S_j}$
\STATE $r_{\Omega_j} \leftarrow A_{\Omega_j,j}$ (Enforce observed ratings)
\ENDFOR
\UNTIL {some stopping criterion is satisfied}
\ENSURE Incomplete predicted rating matrix $R$
\end{algorithmic}
\end{algorithm}

Proof when the number of users goes to infinity:


==> PIM0.tex <==
\newcommand{\p}{\partial}
%\newcommand{\D}{\displaystyle}
\newcommand{\B}{\mathbf}
\newcommand{\M}{\mathcal{M}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bn}{\mathbf{n}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\mathd}{\mathrm{d}}

\newcommand{\bw}{\mathbf{w}}
\newcommand{\bfp}{\mathbf{p}}
\newcommand{\bp}{\mathbf{\Phi}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\al}{\alpha}
\newcommand{\e}{\epsilon}
\newcommand{\Bw}{\mbox{\boldmath$\omega$}}
%\newcommand{\hk}{\exp\left(-\frac{\|\bx-\by\|^2}{4 t}\right)}
%\newcommand{\hkt}{\exp\left(-\frac{\|\bx-\by\|^2}{2 t}\right)}
\newcommand{\hr}{R\left(\frac{|\bx-\by|^2}{4t}\right)}
\newcommand{\hbr}{\bar{R}\left(\frac{|\bx-\by|^2}{4t}\right)}
\newcommand{\nhk}{\frac{1}{(4\pi t)^{k/2}}}
\newcommand{\tnhk}{\frac{1}{(4\pi t)^{k/2}t}}

\newcommand{\bV}{\mathbf{V}}
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\bh}{\mathbf{h}}


\newcommand{\hk}{R_t(\bx, \by)}
\newcommand{\rhk}{\bar{R}_t(\bx, \by)}
\newcommand{\hkpipj}{R_t({\bf p}_i, {\bf p}_j)}
\newcommand{\hkpisj}{R_t({\bf p}_i, {\bf s}_j)}
\newcommand{\rhkpipj}{\bar{R}_t({\bf p}_i, {\bf p}_j)}
\newcommand{\rhkpisj}{\bar{R}_t({\bf p}_i, {\bf s}_j)}
\newcommand{\hkxpj}{R_t(\bx, {\bf p}_j)}
\newcommand{\hkxsj}{R_t(\bx, {\bf s}_j)}
\newcommand{\rhkxpj}{\bar{R}_t(\bx, {\bf p}_j)}
\newcommand{\rhkxsj}{\bar{R}_t(\bx, {\bf s}_j)}
\newcommand{\bff}{{\bf f}}
\newcommand{\bfg}{{\bf g}}
\newcommand{\bfu}{{\bf u}}
%\newcommand{\bfp}{{\bf p}}
\newcommand{\bfs}{{\bf s}}
\newcommand{\bfn}{{\bf n}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bR}{\bar{R}}
\newcommand{\invt}{\frac{1}{t}}
\newcommand{\LP}{\mathcal{L}}
\newcommand{\W}{\mathcal{W}}
\newcommand{\D}{\mathcal{D}}





% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}

\newtheorem{theorem}{\textbf{Theorem}}[section]
\newtheorem{lemma}{\textbf{Lemma}}[section]
\newtheorem{remark}{\textbf{Remark}}[section]
\newtheorem{proposition}{\textbf{Proposition}}[section]
\newtheorem{assumption}{\textbf{Assumption}}[section]
\newtheorem{definition}{\textbf{Definition}}[section]
\newtheorem{corollary}{\textbf{Corollary}}[section]



\noindent {\bf Harmonic Extension:} We consider the harmonic extension in the continuous form, as shown
in Figure \ref{fig:manifold}.
% gives a sketch of the continuous model.
Assume $\M$ is a submanifold embedded in $\mathbb{R}^d$. Consider a function $u(\bx)$
defined on $\M$ and $u(\bx)$ is known in some regions $\Omega_1\cup\cdots\cup\Omega_k\subset\M$.
%For simplicity, we only assume the function $u$ is known in two regions.
%In practical problems, there may be more.
Now, we want to extend the function $u(\bx)$ from
$\Omega_1\cup\cdots \cup\Omega_k$ to the entire manifold $\M$. If the manifold $\M$
has boundary, $\p\M$, we assume $\frac{\p u}{\p \bn}(\bx)=0$ at $\M$.
Then, the harmonic extension problem shown in Figure \ref{fig:manifold} can be modelled as the
following Laplace equation with the mixed boundary condition:
%\begin{equation}
%\left\{
%\begin{array}{rl}
%	-\Delta_\mathcal{M} u(\bx)=0,&\bx\in \mathcal{M}_0\backslash(\Omega_1\cup\Omega_2), \\
%	u(\bx)=g_1(\bx),& \bx\in \p \Omega_1,\\
%       u(\bx)=g_2(\bx),& \bx\in \p \Omega_2,\\
%  \frac{\p u}{\p \bn}(\bx)=0,& \bx \in \p \M_0
%\end{array}
%\right.
%\label{eqn:model}
%\end{equation}
%where $\Delta_{\mathcal{M}}$ is the well-known Laplace-Beltrami operator on $\M$.
\begin{figure}[ht]
  \centering
  \begin{tabular}{cc}
  \includegraphics[width=0.49\textwidth]{./pics/manifold.pdf}
   \end{tabular}
  \caption{Sketch of the manifold.}
  \label{fig:manifold}
\end{figure}
%Generally speaking, harmonic extension amounts to solve the Laplace equation with the following
%mixed boundary condition.
%General model of harmonic extension problem is
% Given a smooth function $g$ over $\p\M$, the harmonic extension $u$ of $g$ in the classical
% sense is the solution to the following Laplace equation with the Dirichlet boundary:
\begin{equation}
\left\{
\begin{array}{rl}
	-\Delta_\mathcal{M} u(\bx)=0,&\bx\in \mathcal{M}, \\
	u(\bx)=g(\bx),& \bx\in \p \mathcal{M}_D,\\
  \frac{\p u}{\p \bn}(\bx)=0,& \bx\in \p \mathcal{M}_N.
\end{array}
\right.
\label{eqn:dirichlet}
\end{equation}
%Here $\M$ and $\p\M$ be a submanifold in $\mathbb{R}^d$ and its boundary respectively,
%and $\p\M=\p\M_D\cup \p\M_N$.
In the aforementioned harmonic extension problem, one can think of $\p\M_D$ as the boundary of
$\Omega_1\cup\cdots \cup\Omega_k$, and $\p\M_N$ as the actual boundary of $\M$.

\noindent{\bf Integral Equation:~}
We observe that the Laplace equation $\Delta \M = 0$ is closely related to the following integral equation.
\begin{align}
\frac{1}{t}\int_{\M} (u(\bx)&-u(\by))w_t(\bx, \by) \mathd \by\nonumber\\ &-2\int_{\p \M} \frac{\p u(\by)}{\p \bn}w_t(\bx, \by) \mathd \tau_\by
 = 0,
\label{eqn:integral}
\end{align}
where $w_t(\bx, \by) = \exp(-\frac{|\bx-\by|^2}{4t})$.

Therefore, we could obtain Theorem~\ref{thm:local-error}, which
follows from the equations~\eqref{eq-integral-part} and \eqref{eq-hessian-euler}.
\begin{theorem}
  \label{thm:local-error}
If $u\in C^3(\M)$ be a harmonic function on $\M$, i.e., $\Delta_\M u =0$,
then we have for any $\bx \in \M$,
\begin{eqnarray}
\label{eqn:local-error}
\left\|r(u) \right\|_{L^2(\mathcal{M})}=O(t^{1/4}).
\end{eqnarray}
where
\begin{align*}
  r(u)=\frac{1}{t}\int_{\M} (u(\bx)&-u(\by))w_t(\bx, \by) \mathd \by \\
&- 2\int_{\p \M} \frac{\p u(\by)}{\p \bn} w_t(\bx, \by) \mathd \tau_\by
\end{align*}
\end{theorem}
The detailed proof can be found in~\cite{SS_neumann}.

\noindent {\bf Dirichlet Boundary:}
Using the integral equation \eqref{eqn:integral} and the boundary condition
of \eqref{eqn:dirichlet}, we know the Laplace equation with the mixed boundary
condition can be approximated by following integral equation:
\begin{align}
\frac{1}{t}\int_{\M} (u(\bx)&-u(\by))w_t(\bx, \by) \mathd \by\nonumber\\ &-2\int_{\p \M_D} \frac{\p u(\by)}{\p \bn}w_t(\bx, \by) \mathd \tau_\by
 = 0,
\label{eqn:integral-mix}
\end{align}
However, on $\p\M_D$, $\frac{\p u}{\p \bn}$ is not known.
To solve this issue, we use the Robin boundary condition to
approximate the original Dirichlet boundary condition on $\p\M_D$.
Then, we consider the following Robin/Neumann mixed boundary problem.
\begin{equation}
\left\{
\begin{array}{rl}
	-\Delta_\mathcal{M} u(\bx)=0,&\bx\in \mathcal{M}, \\
	u(\bx)+\beta \frac{\p u(\bx)}{\p \bn} =g(\bx),& \bx\in \p \mathcal{M}_D,\\
\frac{\p u}{\p \bn}(\bx)=0,& \bx\in \p \mathcal{M}_N.
\end{array}
\right.
\label{eqn:Robin}
\end{equation}
where $\beta>0$ is a parameter.
It is easy to prove that the solution of the above Robin/Neumann problem \eqref{eqn:Robin}
converges to the solution of the Dirichlet/Neumann problem \eqref{eqn:dirichlet}
as $\beta$ goes to 0.

By substituting the Robin boundary $\frac{\p u(\bx)}{\p \bn}=\frac{1}{\beta}(g(\bx)-u(\bx))$
in the integral equation \eqref{eqn:integral-mix}, we get an integral
equation to solve the Robin/Neumann problem.
\begin{align}
\label{eqn:integral-dirichlet}
\frac{1}{t}\int_{\M} (u(\bx)&-u(\by))w_t(\bx, \by) \mathd \by\\ &-\frac{2}{\beta}\int_{\p \M_D} (g(\by)-u(\by))w_t(\bx, \by) \mathd \tau_\by
 = 0, \nonumber
\end{align}
When $\beta>0$ is small enough, this integral equation also gives a good approximation
to the original harmonic extension problem \eqref{eqn:dirichlet}.


\subsection{Discretization}
Denote
\begin{align}
\label{eqn:laplace_op}
L_tu(\bx) &= \frac{1}{t}\int_{\M} (u(\bx)-u(\by)) w_t(\bx, \by) \mathd \by, \\
\label{eqn:bdintegral_op}
I_tu (\bx) &= \int_{\p \M_D} (g(\by)-u(\by)) w_t(\bx, \by) \mathd \tau_\by.
\end{align}
Assume that the point set $X=\{\bx_1, \cdots, \bx_n \}$ samples
the submanifold $\M$ and it is uniformly distributed, then $L_tu$
is discretized and well approximated by $\LP \bu$ up to the volume
weight $\frac{|\M|}{n}$ where $\bu = (u(\bx_1), \cdots, u(\bx_n))$.
Recall that $\LP$ is the weighted graph Laplacian given
in matrix form as $\LP = \frac{1}{t}(\D - \W)$ where $\W=(w_{ij})$ is the weight matrix and
$\D = \mbox{diag}(d_i)$ with $d_i=\sum_j w_{ij}$. In this paper,
we use the Gaussian weight, $w_{ij}=\exp(-\frac{\|\bx_i-\bx_j\|^2}{4t})$.
% If we consider the Laplace equation with the Neumann boundary where $\frac{\p u}{\p \bn} = h$ on $\p\M$ is given,
% we can approximate

The boundary term $I_tu (\bx)$ is actually corresponding to the subset
$B=\{\bb_1,\cdots,\bb_m\}\subset X$ where the values of function $u$ are given.
From the continuous point of view, for each point $\bb_i\in B$, in a
small area around it, the value of $u$ is given. In this sense, each $\bb_i$
actually stands for one part of the boundary $\p\M_D$. Based on the
above discussion, the boundary term $I_tu (\bx)$  can be discretized
as $\sum_{\bb_i\in B} w_t(\bx, \bb_i) (g(\bb_i)-u(\bb_i))$
up to the surface area weight $\frac{|\p\M_D|}{m}$.% , provided that the point set
% $B=(\bb_1, \cdots, \bb_m) \subset X$ samples $\p\M$ and is uniformly distributed also.

% Then we can discretize the integral equation~\eqref{eqn:integral} using the linear system
% \begin{equation}
% \LP \bu - 2\frac{n|\p\M|}{m|\M|}\W(X, B) \bh = 0,
% \end{equation}
% where $\bh = (h(\bb_1), \cdots, h(\bb_m))$.
% We now use the Robin boundary $u + \beta  \frac{\p u(\by)}{\p \bn} = g$ on $\p\M$ to bridge
% the Dirichlet boundary and the Neumann boundary as follows.
% For a small parameter $\beta$, the above Robin boundary approximates the Dirichlet boundary $u=g$ on $\p\M$.
% At the same time, we can write the Neumann boundary $\frac{\p u}{\p \bn} = \frac{1}{\beta} (g - u_B)$.
Therefore, the harmonic extension problem~\eqref{eqn:dirichlet} can be numerically solved
by the following linear system
%~\eqref{eqn:dirichlet_dis} if set $\mu =  \frac{2}{\beta}\frac{|\M|}{|\p\M|}$.
\begin{equation}
\LP \bu - \frac{2}{\beta}\frac{n|\p\M_D|}{m|\M|}\W(X, B) (\bg - \bu_B) = 0
\label{eqn:dirichlet_dis_1}
\end{equation}
where $\W(X, B)$ is a submatrix of the weight matrix $\W$ by taking the columns corresponding to
the subset $B$, and $\bg=(g(\bb_1),\cdots, g(\bb_{m}))$ and $\bu_B=(u(\bb_1),\cdots,u(\bb_m))$.
This is the same as the linear system~\eqref{eqn:dirichlet_dis} if
set $\mu =  \frac{2}{\beta}\frac{n|\p\M_D|}{m|\M|}$.
In the examples shown in the paper,  we take
$\beta = 10^{-4}\frac{|\p\M_D|}{|\M|} $, and thus $\mu = 10^4\frac{n}{m}$.

When the points $X$ and $B$ uniform randomly
sample a submanifold and its boundary respectively in the iid fashion, the harmonic function
computed by PIM is guaranteed to converge to the one in the classical sense. For the details of the
theoretical analysis, we refer to \cite{SS_neumann,SS_dirichlet}.



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper0104"
%%% End:


==> PIM1.tex <==
\newcommand{\p}{\partial}
%\newcommand{\D}{\displaystyle}
\newcommand{\B}{\mathbf}
\newcommand{\M}{\mathcal{M}}

\newcommand{\mathd}{\mathrm{d}}

\newcommand{\bw}{\mathbf{w}}
\newcommand{\bfp}{\mathbf{p}}
\newcommand{\bp}{\mathbf{\Phi}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\al}{\alpha}
\newcommand{\e}{\epsilon}
\newcommand{\Bw}{\mbox{\boldmath$\omega$}}
%\newcommand{\hk}{\exp\left(-\frac{\|\bx-\by\|^2}{4 t}\right)}
%\newcommand{\hkt}{\exp\left(-\frac{\|\bx-\by\|^2}{2 t}\right)}
\newcommand{\hr}{R\left(\frac{|\bx-\by|^2}{4t}\right)}
\newcommand{\hbr}{\bar{R}\left(\frac{|\bx-\by|^2}{4t}\right)}
\newcommand{\nhk}{\frac{1}{(4\pi t)^{k/2}}}
\newcommand{\tnhk}{\frac{1}{(4\pi t)^{k/2}t}}

\newcommand{\bV}{\mathbf{V}}
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\bh}{\mathbf{h}}


\newcommand{\hk}{R_t(\bx, \by)}
\newcommand{\rhk}{\bar{R}_t(\bx, \by)}
\newcommand{\hkpipj}{R_t({\bf p}_i, {\bf p}_j)}
\newcommand{\hkpisj}{R_t({\bf p}_i, {\bf s}_j)}
\newcommand{\rhkpipj}{\bar{R}_t({\bf p}_i, {\bf p}_j)}
\newcommand{\rhkpisj}{\bar{R}_t({\bf p}_i, {\bf s}_j)}
\newcommand{\hkxpj}{R_t(\bx, {\bf p}_j)}
\newcommand{\hkxsj}{R_t(\bx, {\bf s}_j)}
\newcommand{\rhkxpj}{\bar{R}_t(\bx, {\bf p}_j)}
\newcommand{\rhkxsj}{\bar{R}_t(\bx, {\bf s}_j)}
\newcommand{\bff}{{\bf f}}
\newcommand{\bfg}{{\bf g}}
\newcommand{\bfu}{{\bf u}}
%\newcommand{\bfp}{{\bf p}}
\newcommand{\bfs}{{\bf s}}
\newcommand{\bfn}{{\bf n}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bR}{\bar{R}}
\newcommand{\invt}{\frac{1}{t}}
\newcommand{\LP}{\mathcal{L}}
\newcommand{\W}{\mathcal{W}}
\newcommand{\D}{\mathcal{D}}





% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}

\newtheorem{theorem}{\textbf{Theorem}}[section]
\newtheorem{lemma}{\textbf{Lemma}}[section]
\newtheorem{remark}{\textbf{Remark}}[section]
\newtheorem{proposition}{\textbf{Proposition}}[section]
\newtheorem{assumption}{\textbf{Assumption}}[section]
\newtheorem{definition}{\textbf{Definition}}[section]
\newtheorem{corollary}{\textbf{Corollary}}[section]





\paragraph{Integral Equation:~}
The key observation in PIM is that the Laplace-Beltrami operator has the following integral approximation:
\begin{align}
&\int_{\M}w_t(\bx,\by)\Delta_{\M}f(\by)\mathd \by\nonumber
\\\approx &
-\frac{1}{t}\int_{\M} (f(\bx)-f(\by))w_t(\bx, \by) \mathd \by\nonumber\\
&+2\int_{\p \M} \frac{\p u(\by)}{\p \bn}w_t(\bx, \by) \mathd \tau_\by,
\label{eqn:integral}
\end{align}
where $w_t(\bx, \by) = \exp(-\frac{|\bx-\by|^2}{4t})$. The following theorem gives the accuracy of the integral approximation.
\begin{theorem}
  \label{thm:local-error} \cite{neumann}
If $f\in C^3(\M)$ is a smooth function on $\M$,
then for any $\bx \in \M$,
\begin{eqnarray}
\label{eqn:local-error}
\left\|r(u) \right\|_{L^2(\mathcal{M})}=O(t^{1/4}),
\end{eqnarray}
where
\begin{align*}
  r(u)=&\int_{\M}w_t(\bx,\by)\Delta_{\M}f(\by)\mathd \by\\
&+\frac{1}{t}\int_{\M} (u(\bx)-u(\by))w_t(\bx, \by) \mathd \by \\
&- 2\int_{\p \M} \frac{\p u(\by)}{\p \bn} w_t(\bx, \by) \mathd \tau_\by.
\end{align*}
\end{theorem}
%The detailed proof can be found in~\cite{SS_neumann}.
Applying the integral approximation \eqref{eqn:integral} to the Laplace-Beltrami equation \eqref{laplace}, we get an 
integral equation
\begin{align}
\frac{1}{t}\int_{\M} (f(\bx)&-f(\by))w_t(\bx, \by) \mathd \by\nonumber\\
&+\mu\sum_{\by\in \Lambda}w_t(\bx,\by)(f(\by)-h(\by))= 0,
\label{eqn:integral2}
\end{align}
In this integral equation, there are no derivatives, and therefore it is easy to discretize over the point cloud. 

\paragraph{Discretization}
We notice that the closed form of the user manifold $\M$ is not known, and we only have a sample of $\M$, i.e. $U$.
Next, we discretize the integral equation \eqref{eqn:integral} over the point set $U$. 

Assume that the point set $U$ is uniformly distributed over $\M$. The integral equation can be 
discretized easily, as follows: 
\begin{align}
  \label{eq:discretize}
  \frac{|\M|}{m}\sum_{j=1}^m &w_t(\bx_i,\bx_j)(f(\bx_i)-f(\bx_j))+\nonumber\\
&\mu t \sum_{\by\in \Lambda}w_t(\bx_i,\by)(f(\by)-h(\by))=0
\end{align}
where $|\M|$ is the volume of the manifold $\M$.

We can rewrite \eqref{eq:discretize} in the matrix form.
\begin{align}
  \label{eq:dis-matrix}
  \bm{L}\bm{f}+\bar{\mu} \bm{W}_{:,\Lambda}\bm{f}_\Lambda=\bar{\mu} \bm{W}_{:,\Lambda}\bm{h}.
\end{align}
where $\bm{h}=(h_1,\cdots,h_m)$ and $\bar{\mu}=\frac{\mu t m}{|\M|}$. $\bm{L}$ is a $m\times m$ matrix which is given as
% then $L_tu$ 
% is discretized and well approximated by $\mathcal{L} \bu$ up to the volume weight $\frac{|\M|}{n}$ where $\bu = (u(\bx_1), \cdots, u(\bx_n))$. 
% Remeber that $\mathcal{L}$ is the weighted graph Laplacian given 
% in matrix form as $\mathcal{L} = \frac{1}{t}(\mathcal{D} - \mathcal{W})$ In this paper, we use the Gaussian weight, $w_{ij}=\exp(-\frac{\|\bx_i-\bx_j\|^2}{4t})$.
\begin{align}
  \label{eq:matrix-L}
  \bm{L}=\bm{D}-\bm{W}
\end{align}
 where $\bm{W}=(w_{ij}),\; i,j=1,\cdots, m$ is the weight matrix and 
$\bm{D} = \mbox{diag}(d_i)$ with $d_i=\sum_{j=1}^m w_{ij}$.
%$\bm{W}(U, \Lambda)$ is a submatrix of the weight matrix $\bm{W}$ by taking the columns corresponding to the subset $\Lambda$.


\begin{algorithm}[tb]
\floatname{algorithm}{Algorithm}
\caption{Harmonic Extension}
\label{alg:harmonic}
\begin{algorithmic}[1]
\REQUIRE Initial rating matrix $A$.
\ENSURE  Rating matrix $R$.
\STATE Set $R=A$.
\REPEAT
\STATE Estimate the weight matrix $\bm{W}=(w_{ij})$ from the user set $U$ (Algorithm \ref{alg:sim_matrix}).
%\STATE Assemble the matrices $\bm{L}$ and $\bm{W}$ as follows:
%\begin{align*}
%  \bm{L}=\bm{D}-\bm{W}, \; \bm{W}=(w_{ij}),\; i,j=1,\cdots, m.
%\end{align*}
\STATE Compute the graph Laplacian matrix: $\bm{L}=\bm{D}-\bm{W}$
\FOR{$i=1$ to $n$}
\REPEAT
\STATE Solve the following linear systems
\begin{align*}
  \bm{L}\bm{f}_i+\bar{\mu} \bm{W}_{:,U_i}(\bm{f}_i)_{U_i}=\bar{\mu} \bm{W}_{:,U_i}\bm{h}_{U_i},
\end{align*}
where $\bm{h}=g-d^n$.
\STATE Update $d^n$,
$$d^{n+1}=d^n+f^{n+1}-g$$
\UNTIL {some stopping criterion for the Bregman iterations is satisfied} 
\ENDFOR
\STATE $r_{ij}=f_i(u_j)$ and $R=(r_{ij})$.
\UNTIL {some stopping criterion is satisfied}
\end{algorithmic}
\end{algorithm}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper0104"
%%% End:


==> PIM2.tex <==
\newcommand{\p}{\partial}
%\newcommand{\D}{\displaystyle}
\newcommand{\B}{\mathbf}
\newcommand{\M}{\mathcal{M}}

\newcommand{\mathd}{\mathrm{d}}

\newcommand{\bw}{\mathbf{w}}
\newcommand{\bfp}{\mathbf{p}}
\newcommand{\bp}{\mathbf{\Phi}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\al}{\alpha}
\newcommand{\e}{\epsilon}
\newcommand{\Bw}{\mbox{\boldmath$\omega$}}
%\newcommand{\hk}{\exp\left(-\frac{\|\bx-\by\|^2}{4 t}\right)}
%\newcommand{\hkt}{\exp\left(-\frac{\|\bx-\by\|^2}{2 t}\right)}
\newcommand{\hr}{R\left(\frac{|\bx-\by|^2}{4t}\right)}
\newcommand{\hbr}{\bar{R}\left(\frac{|\bx-\by|^2}{4t}\right)}
\newcommand{\nhk}{\frac{1}{(4\pi t)^{k/2}}}
\newcommand{\tnhk}{\frac{1}{(4\pi t)^{k/2}t}}

\newcommand{\bV}{\mathbf{V}}
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\bh}{\mathbf{h}}


\newcommand{\hk}{R_t(\bx, \by)}
\newcommand{\rhk}{\bar{R}_t(\bx, \by)}
\newcommand{\hkpipj}{R_t({\bf p}_i, {\bf p}_j)}
\newcommand{\hkpisj}{R_t({\bf p}_i, {\bf s}_j)}
\newcommand{\rhkpipj}{\bar{R}_t({\bf p}_i, {\bf p}_j)}
\newcommand{\rhkpisj}{\bar{R}_t({\bf p}_i, {\bf s}_j)}
\newcommand{\hkxpj}{R_t(\bx, {\bf p}_j)}
\newcommand{\hkxsj}{R_t(\bx, {\bf s}_j)}
\newcommand{\rhkxpj}{\bar{R}_t(\bx, {\bf p}_j)}
\newcommand{\rhkxsj}{\bar{R}_t(\bx, {\bf s}_j)}
\newcommand{\bff}{{\bf f}}
\newcommand{\bfg}{{\bf g}}
\newcommand{\bfu}{{\bf u}}
%\newcommand{\bfp}{{\bf p}}
\newcommand{\bfs}{{\bf s}}
\newcommand{\bfn}{{\bf n}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bR}{\bar{R}}
\newcommand{\invt}{\frac{1}{t}}
\newcommand{\LP}{\mathcal{L}}
\newcommand{\W}{\mathcal{W}}
\newcommand{\D}{\mathcal{D}}





% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}

\newtheorem{theorem}{\textbf{Theorem}}[section]
\newtheorem{lemma}{\textbf{Lemma}}[section]
\newtheorem{remark}{\textbf{Remark}}[section]
\newtheorem{proposition}{\textbf{Proposition}}[section]
\newtheorem{assumption}{\textbf{Assumption}}[section]
\newtheorem{definition}{\textbf{Definition}}[section]
\newtheorem{corollary}{\textbf{Corollary}}[section]





\paragraph{Integral Equation:~}
The key observation in PIM is that the Laplace-Beltrami operator has the following integral approximation:
\begin{align}
&\int_{\M}w_t(\bx,\by)\Delta_{\M}f(\by)\mathd \by\nonumber
\\\approx &
-\frac{1}{t}\int_{\M} (f(\bx)-f(\by))w_t(\bx, \by) \mathd \by\nonumber\\
&+2\int_{\p \M} \frac{\p u(\by)}{\p \bn}w_t(\bx, \by) \mathd \tau_\by,
\label{eqn:integral}
\end{align}
where $w_t(\bx, \by) = \exp(-\frac{|\bx-\by|^2}{4t})$. The following theorem gives the accuracy of the integral approximation.
\begin{theorem}
  \label{thm:local-error} \cite{neumann}
If $f\in C^3(\M)$ is a smooth function on $\M$,
then for any $\bx \in \M$,
\begin{eqnarray}
\label{eqn:local-error}
\left\|r(u) \right\|_{L^2(\mathcal{M})}=O(t^{1/4}),
\end{eqnarray}
where
\begin{align*}
  r(u)=&\int_{\M}w_t(\bx,\by)\Delta_{\M}f(\by)\mathd \by\\
&+\frac{1}{t}\int_{\M} (u(\bx)-u(\by))w_t(\bx, \by) \mathd \by \\
&- 2\int_{\p \M} \frac{\p u(\by)}{\p \bn} w_t(\bx, \by) \mathd \tau_\by.
\end{align*}
\end{theorem}
%The detailed proof can be found in~\cite{SS_neumann}.
Applying the integral approximation \eqref{eqn:integral} to the Laplace-Beltrami equation \eqref{laplace}, we get an 
integral equation
\begin{align}
\frac{1}{t}\int_{\M} (f(\bx)&-f(\by))w_t(\bx, \by) \mathd \by\nonumber\\
&+\mu\sum_{\by\in \Lambda}w_t(\bx,\by)(f(\by)-h(\by))= 0,
\label{eqn:integral2}
\end{align}
In this integral equation, there are no derivatives, and therefore it is easy to discretize over the point cloud. 

\paragraph{Discretization}
We notice that the closed form of the user manifold $\M$ is not known, and we only have a sample of $\M$, i.e. $U$.
Next, we discretize the integral equation \eqref{eqn:integral} over the point set $U$. 

Assume that the point set $U$ is uniformly distributed over $\M$. The integral equation can be 
discretized easily, as follows: 
\begin{align}
  \label{eq:discretize}
  \frac{|\M|}{m}\sum_{j=1}^m &w_t(\bx_i,\bx_j)(f(\bx_i)-f(\bx_j))+\nonumber\\
&\mu t \sum_{\by\in \Lambda}w_t(\bx_i,\by)(f(\by)-h(\by))=0
\end{align}
where $|\M|$ is the volume of the manifold $\M$.

We can rewrite \eqref{eq:discretize} in the matrix form.
\begin{align}
  \label{eq:dis-matrix}
  \bm{L}\bm{f}+\bar{\mu} \bm{W}_{:,\Lambda}\bm{f}_\Lambda=\bar{\mu} \bm{W}_{:,\Lambda}\bm{h}.
\end{align}
where $\bm{h}=(h_1,\cdots,h_m)$ and $\bar{\mu}=\frac{\mu t m}{|\M|}$. $\bm{L}$ is a $m\times m$ matrix which is given as
% then $L_tu$ 
% is discretized and well approximated by $\mathcal{L} \bu$ up to the volume weight $\frac{|\M|}{n}$ where $\bu = (u(\bx_1), \cdots, u(\bx_n))$. 
% Remeber that $\mathcal{L}$ is the weighted graph Laplacian given 
% in matrix form as $\mathcal{L} = \frac{1}{t}(\mathcal{D} - \mathcal{W})$ In this paper, we use the Gaussian weight, $w_{ij}=\exp(-\frac{\|\bx_i-\bx_j\|^2}{4t})$.
\begin{align}
  \label{eq:matrix-L}
  \bm{L}=\bm{D}-\bm{W}
\end{align}
 where $\bm{W}=(w_{ij}),\; i,j=1,\cdots, m$ is the weight matrix and 
$\bm{D} = \mbox{diag}(d_i)$ with $d_i=\sum_{j=1}^m w_{ij}$.
%$\bm{W}(U, \Lambda)$ is a submatrix of the weight matrix $\bm{W}$ by taking the columns corresponding to the subset $\Lambda$.


\begin{algorithm}[tb]
\floatname{algorithm}{Algorithm}
\caption{Harmonic Extension}
\label{alg:harmonic}
\begin{algorithmic}[1]
\REQUIRE Initial rating matrix $A$.
\ENSURE  Rating matrix $R$.
\STATE Set $R=A$.
\REPEAT
\STATE Estimate the weight matrix $\bm{W}=(w_{ij})$ from the user set $U$ (Algorithm \ref{alg:sim_matrix}).
%\STATE Assemble the matrices $\bm{L}$ and $\bm{W}$ as follows:
%\begin{align*}
%  \bm{L}=\bm{D}-\bm{W}, \; \bm{W}=(w_{ij}),\; i,j=1,\cdots, m.
%\end{align*}
\STATE Compute the graph Laplacian matrix: $\bm{L}=\bm{D}-\bm{W}$
\FOR{$i=1$ to $n$}
\REPEAT
\STATE Solve the following linear systems
\begin{align*}
  \bm{L}\bm{f}_i+\bar{\mu} \bm{W}_{:,U_i}(\bm{f}_i)_{U_i}=\bar{\mu} \bm{W}_{:,U_i}\bm{h}_{U_i},
\end{align*}
where $\bm{h}=g-d^n$.
\STATE Update $d^n$,
$$d^{n+1}=d^n+f^{n+1}-g$$
\UNTIL {some stopping criterion for the Bregman iterations is satisfied} 
\ENDFOR
\STATE $r_{ij}=f_i(u_j)$ and $R=(r_{ij})$.
\UNTIL {some stopping criterion is satisfied}
\end{algorithmic}
\end{algorithm}

\begin{remark}
  In the harmonic extension approach, we use a continuous formulation based on the underlying user manifold. And the point integral method is used to 
solve the Laplace-Beltrami equation on the manifold. If the graph model was used at the beginning, the natural choice to do the harmonic extension is the graph Laplacian. 
However, it has been observed that the graph Laplacian is not consisitent in solving the harmonic extension problem \cite{harmonic,LDMM_image}. PIM gives much better results. 
\end{remark}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper0201"
%%% End:


==> experiments.tex <==
In this section, we evaluate our proposed method LDM in terms of both run-time and ranking quality. Since the volume of literature on recommender systems, collaborative filtering, and matrix completion is huge, we select only a few existing methods to compare with. All the experiments are run on a Linux laptop with one Intel i7-5600U CPU (4 physical threads) and 8 GB memory.

\subsection{Data Sets}

We use three MovieLens\footnote{\url{http://grouplens.org/datasets/movielens/}} data sets in our experiments: {\em MovieLens-100k}, {\em MovieLens-1m}, and {\em MovieLens-10m}. In each of the data sets, each user has at least 20 ratings. Following the convention in previous work on collaborative ranking, we randomly select $N$ ratings for each user as the training set, and the other ratings were used for testing. To keep at least 10 ratings in the testing set for each user, we remove the users with fewer than $N+10$ ratings. After this preprocessing, we can generate several versions of these data sets with different $N$'s, whose information is summarized in Table \ref{table:datasets}.

\subsection{Methods for Comparison}
\label{algcompare}

\begin{figure*}[!t]
\vskip 0.1in
\includegraphics[width=0.33\textwidth]{kdtree_ml100k_N_10}
\includegraphics[width=0.33\textwidth]{kdtree_ml100k_N_20}
\includegraphics[width=0.33\textwidth]{kdtree_ml1m_N_20}
\caption{Ranking quality NDCG@$10$ (Section \ref{sec:eval_measure}) as a function of the number of nearest neighbors ($k$) when constructing the {\em kd}-tree and the maximum number of comparisons ($D$) when querying the {\em kd}-tree. $k$ must not be larger than $D$.}
\label{fig:kdtree_param} \centering
\vskip -0.1in
\end{figure*}

\begin{figure*}[!t]
\vskip 0.1in
\includegraphics[width=0.32\textwidth]{ml100k_N_10}
\includegraphics[width=0.34\textwidth]{ml100k_N_20}
\includegraphics[width=0.325\textwidth]{ml1m_N_20}
\caption{Ranking quality NDCG@$10$ (Section \ref{sec:eval_measure}) vs. run-time under various hyperparameters for each of the methods compared. LCR and SVD are time-consuming and therefore their results with multiple sets of hyperparameters are not available on MovieLens-1m.}
\label{fig:all_param} \centering
\vskip -0.2in
\end{figure*}

We compare our LDM method with singular value decomposition (SVD) as a baseline, and two state-of-the-art methods that are designed specifically for collaborative ranking. All the three methods for comparison optimize a pairwise ranking loss function. We do not perform hyperparameter selection on a separate validation set because it is time-consuming, but we investigate the effect of the hyperparameters in Section \ref{hyperparameters}; and in Section \ref{results}, we use a fixed set of hyperparameters that can achieve a good balance between run-time and ranking quality, which are found empirically across several data sets. We list these methods below (their program options that will be used in Section \ref{results} is in the footnote):
\begin{itemize}
\item {\em SVD}: We use the Java implementation of ranking-based SVD in the PREA toolkit\footnote{\url{http://prea.gatech.edu}}$^,$\footnote{The command-line options for SVD is \texttt{-a ranksvd exp\_add 5 5 25}.}. This version uses gradient descent to optimize the ranking-based loss function (\ref{pairwiseloss}), as opposed to the squared loss function in regularized SVD.
\item {\em LCR}: Local collaborative ranking \cite{lcr}, as implemented in the PREA toolkit\footnote{The command-line options for LCR is \texttt{-a pgllorma exp\_add 5 5 13}.}.
\item {\em AltSVM}: Alternating support vector machine \cite{altsvm}, as implemented in the \texttt{collranking} package\footnote{\url{https://github.com/dhpark22/collranking}}. We employ the default configurations.
\end{itemize}

\begin{table}[!t]
\caption{Statistics of the data sets in our experiments. $N$ is the number of ratings in the training set for each user. The total number of ratings in the training set is $N\times$(\# users).}
\label{table:datasets} \centering
\vskip 0.15in
{\small
\begin{tabular}{|l|c|r|r|r|}
\hline
\multicolumn{2}{|c|}{Data set} & \# users & \# items & \# ratings \\
\hline
\multirow{2}{*}{MovieLens-100k} & $N=10$ & 943 & 1,682 & 100,000 \\
 & $N=20$ & 744 & 1,682 & 95,269 \\
\hline
\multirow{3}{*}{MovieLens-1m} & $N=10$ & 6,040 & 3,706 & 1,000,209 \\
 & $N=20$ & 5,289 & 3,701 & 982,040 \\
 & $N=50$ & 3,938 & 3,677 & 924,053 \\
\hline
\multirow{4}{*}{MovieLens-10m} & $N=10$ & 69,878 & 10,677 & 10,000,054 \\
& $N=20$ & 57,534 & 10,675 & 9,704,223 \\
& $N=50$ & 38,604 & 10,672 & 8,897,688 \\
 & $N=100$ & 24,328 & 10,666 & 7,730,011 \\
\hline
\end{tabular}}
\vskip -0.1in
\end{table}

Lastly, our proposed method LDM (Algorithm \ref{alg:harmonic}) is implemented in Matlab, and the construction and querying of the {\em kd}-tree (Algorithm \ref{alg:sim_matrix}) is implemented in C, for which we extended the VLFeat\footnote{\url{http://www.vlfeat.org/}} package to build a {\em kd}-tree with a sparse input matrix efficiently. In Algorithm \ref{alg:harmonic}, we set $\mu=1$ and run one inner iteration and one outer iteration only, since we empirically found that the weight matrix constructed from the incomplete input ratings by Algorithm \ref{alg:sim_matrix} is often good enough for the algorithm to converge in one iteration. Algorithm \ref{alg:harmonic} typically accounts for most ($\sim95$\%) of the run-time in our method.

All the programs except SVD use 4 threads in our experiments, and are applied to the same training and testing random splits.

\subsection{Evaluation Measure}
\label{sec:eval_measure}

We evaluate the ranking quality by {\em normalized discounted cumulative gain} (NDCG) @$K$ \cite{ndcg}, averaged over all the users. Given a ranked list of $t$ items $i_1,\cdots,i_t$ and their {\em ground-truth} relevance score $r_{i_1},\cdots,r_{i_t}$, the DCG@$K$ score ($K \leq t$) is computed as
\begin{equation}
\label{dcg}
\text{DCG@}K (i_1,\cdots,i_t) = \sum_{j=1}^K {2^{r_{i_j}} - 1 \over \log_2(j+1)}.
\end{equation}
Then, we sort the list of items in the decreasing order of the relevance score and obtain the list $i_1^*,\cdots,i_t^*$, where $r_{i_1^*} \geq \cdots \geq r_{i_t^*}$, and this sorted list achieves the maximum DCG@$K$ score over all the possible permutations. The NDCG score is defined as the normalized version of (\ref{dcg}):
\begin{equation}
\label{ndcg}
\text{NDCG@}K (i_1,\cdots,i_t) = {\text{DCG@}K (i_1,\cdots,i_t) \over \text{DCG@}K (i_1^*,\cdots,i_t^*)}.
\end{equation}
We only evaluate NDCG@$10$ due to limited space. Note that for a user $u$, the list of items that is provided to compute (\ref{ndcg}) is {\em all} the items with observed ratings given by $u$ in the test set, not only the highest-ranking ones.

In contrast to previous work on top-N recommender systems \cite{eval_topn,eval_topn2}, we discourage the use of Precision@$K$ in the context of collaborative ranking for recommender systems, which measures the proportion of actually rated items out of the top $K$ items in the ranked list of all the items in the data set. Contemporary recommender systems typically use numeric ratings rather than binary ratings. In a 1-to-5 rating system, for example, a 1-star item should be less favorable than an unrated item with an expected 3-star rating. However, a recommender system that ranks 1-star items at the top positions would get a higher Precision@$K$ score than one that ranks unrated items at the top positions. Thus, Precision@$K$ is not a valid measure for collaborative ranking with a non-binary rating system.

%For measuring the run-time, we take both the training and testing phases into account, because both phases are important for evaluating the computational efficiency of a real recommender system. In the testing phase, a real system has to compute the ratings for all the items and return the top-rated ones to the user, whereas we only include the time for computing the ratings in the test set.

\subsection{Effect of Parameter Selection}
\label{hyperparameters}

\begin{table*}[!t]
\caption{Benchmarking results of ranking quality NDCG@$10$ (Section \ref{sec:eval_measure}) and run-time for all the compared methods. $N$ is the number of ratings in the training set for each user.
%``n/a'' indicates the methods that did not finish within a few hours.
}
\label{table:final_result} \centering
\vskip 0.15in
{\small
\begin{tabular}{|l||c|c|c|c||r|r|r|r|}
\hline
\multirow{2}{*}{} & \multicolumn{4}{c||}{\textbf{NDCG@$10$}} & \multicolumn{4}{c|}{\textbf{Time (seconds)}} \\
\cline{2-9} & SVD & LCR & AltSVM & LDM & SVD & LCR & AltSVM & LDM \\
\hline
MovieLens-1m, $N=10$ & 0.6836 & 0.7447 & 0.6680 & 0.7295 & 844.4 & 254.2 & 3.6 & 61.1 \\
\hline
MovieLens-1m, $N=20$ & 0.6758 & 0.7428 & 0.6879 & 0.7404 & 843.3 & 437.3 & 6.8 & 52.3 \\
\hline
MovieLens-1m, $N=50$ & 0.6178 & 0.7470 & 0.7730 & 0.7527 & 730.5 & 1168.8 & 53.0 & 37.0 \\
\hline
MovieLens-10m, $N=10$ & 0.6291 & 0.6866 & 0.6536 & 0.7077 & 24913.4 & 4544.4 & 61.2 & 1496.3 \\
\hline
MovieLens-10m, $N=20$ & 0.6201 & 0.6899 & 0.7208 & 0.7213 & 14778.5 & 6823.5 & 275.4 & 1653.1 \\
\hline
MovieLens-10m, $N=50$ & 0.5731 & 0.6830 & 0.7507 & 0.7286 & 10899.1 & 14668.5 & 648.4 & 1295.0 \\
\hline
MovieLens-10m, $N=100$ & 0.5328 & 0.7125 & 0.7719 & 0.7349 & 14648.5 & 4289.1 & 1411.2 & 832.0 \\
\hline
\end{tabular}}
\vskip -0.1in
\end{table*}

First, we examine the influence of the {\em kd}-tree parameters on the performance of LDM, namely the number of nearest neighbors $k$ and the maximum number of distance comparisons $D$. Fig. \ref{fig:kdtree_param} shows the change in NDCG@$10$ when varying $k$ and $D$ on several small data sets (due to time constraints). In general, the ranking quality is much better with moderately large $k,D$ values than with very small $k,D$ values, but does not improve much when further increasing $k$ and $D$. Therefore, we can use sufficiently large $k,D$ values to get good ranking quality, but not too large to be computationally efficient. In the experimental comparison in Section \ref{results}, we fix the parameters to $k=64$ and $D=256$.

Next, we vary the hyperparameters in each of the four methods, and compare simultaneously the ranking quality and run-time under different hyperparameters. Ideally, a good performance of a collaborative ranking method means producing higher NDCG@$10$ scores in less time. Fig. \ref{fig:all_param} plots NDCG@$10$ against the run-time for several small data sets (due to time constraints). LDM achieves the highest NDCG@$10$ in a reasonable amount of time compared to the other methods. AltSVM is efficient but produces unsatisfactory ranking quality, which is also sensitive to its hyperparameters. For LCR, the ranking quality is acceptable but it takes considerably longer time, especially when the size of training set increases. On MovieLens-100k ($N=20$), SVD and LDM achieve similar NDCG@$10$ scores but LDM costs much shorter run-time.

\subsection{Results}
\label{results}

Now we fix the hyperparameters as described in Section \ref{algcompare}. Table \ref{table:final_result} reports the run-time and NDCG@$10$ scores for all the compared methods on the larger data sets. LDM does not achieve the highest NDCG@$10$ scores in every case, but produces robust ranking quality with decent run-time (except MovieLens-10m, $N=50$). For LCR and SVD, the time cost increases dramatically on larger data sets. AltSVM achieves superior ranking quality when the number of training ratings $N$ is large, but its performance is sensitive to the number of iterations, which in turn depends on the data set and the given tolerance parameter. We conclude that LDM is an overall competitive method that is efficient and robust to hyperparameters and the underlying data sets. Also, LDM has particular advantages when the available information is relatively few, i.e. when $N$ is small, which we consider is a more difficult problem than the cases with richer training information.

We can clearly see that the run-time of LDM increases with the number of users (due to the reliance on the user-user similarity matrix, as expected), while the run-time of AltSVM increases with the number of ratings in the training set. Further optimizing the code for LDM is an important direction in our future work to make it efficient for large-scale data sets.

We note that our method predicts all the missing ratings in the label propagation process, which is included in the timing of LDM, and therefore our methods takes a negligible amount of time for testing, especially in the real scenario where a recommendation algorithm would have to predict the ratings for all the items and return the top-rated ones to the user.
%Also, our method can be fully parallelized on distributed machines, since the linear systems that need to be solved for all the items are independent with one another.


==> harmonic0.tex <==
Consider an user-by-item rating matrix $A \in \mathbb{R}^{m \times n}$, where rows correspond to $m$ users, and columns correspond to $n$ items. The observed ratings are indexed by the set $\Omega=\{(i,j) : \text{user }i\text{ rated item }j\}$. The goal is to predict the missing entries that are not in $\Omega$. Let our current estimate of the ratings be a matrix $R \in \mathbb{R}^{m \times n}$ (may be incomplete), and initially $R=A$. Suppose there exists a ``true'' rating matrix $A^*$ given by an oracle with no missing entries, which is not known to us, and $A|_{\Omega} = A^*|_{\Omega}$. Without loss of generality, we consider the rows of $A^*$ as data points.

We define the harmonic extension problem that solves the matrix completion problem in a continuous setting. Imaging there exists an user-by-item rating system with infinite
number of users. With fixed items,
each users is represented by a $n$-dimensional vector consisted of the rating to $n$ items. The whole user-by-item rating matrix, $A$, is equivalent to
a point set $\mathcal{C}(A)$ in $\mathbb{R}^n$. Imaging that the number of users tends to infinity, we assume that $\mathcal{C}(A)$ becomes a submanifold embedded
in $\mathbb{R}^n$.
Let users be sampled from a manifold $\mathcal{M} \subset \mathbb{R}^n$, and define a real-valued function $f: \mathcal{M}^n \rightarrow \mathbb{R}$ that maps a user into the rating of some particular item. We know the function values at the points in $\partial \mathcal{M}$ (boundary condition): $f(u)|_{\partial \mathcal{M}}=g(u)$, and would like to obtain $f(u)|_{\mathcal{M} \backslash \partial \mathcal{M}}$. Thus, this can be viewed as a semi-supervised regression problem.

It is natural to define the following energy functional:
\begin{equation}
\label{energy}
E(f) = \int_{\mathcal{M}} \|\nabla f_{\mathcal{M}}(u)\|^2 du,
\end{equation}
where $\nabla f_{\mathcal{M}}(u)$ is the nonlocal gradient at $u$ defined on the manifold. Solving the energy minimization problem
\begin{equation}
\label{minenergy}
\min_f E(f) \text{  subject to  } f(u)|_{\partial \mathcal{M}}=g(u)
\end{equation}
will encourage similar users to have similar ratings for this item. Eq. (\ref{minenergy}) is the problem we focus on.

It is well known that the solution to (\ref{minenergy}) can be reduced to the following Laplace equation with Dirichlet boundary:
\begin{equation}
\label{laplace}
\begin{cases}
\Delta_{\mathcal{M}} f(u) = 0, \quad u \in \mathcal{M} \backslash \partial \mathcal{M}, \\
f(u)=g(u), \quad u \in \partial \mathcal{M},
\end{cases}
\end{equation}
which is to say, the function $f$ that minimizes (\ref{minenergy}) is a harmonic function on $\mathcal{M} \backslash \partial \mathcal{M}$. Thus, (\ref{laplace}) is called the {\em harmonic extension} problem in the continuous setting.

Now we will extend the above theory to predict the ratings for all the items in a data set. Let us use $f_1,f_2,\cdots,f_n: \mathcal{M} \rightarrow \mathbb{R}$ to denote the functions that map a user to the ratings of item $1$, item $2$, $\cdots$, item $n$, respectively.

We consider the energy minimization problems
\begin{equation}
\label{minenergy_all}
\min_{f_j} E(f_j) \text{  subject to  } f_j(u)|_{\Omega_j}=g_j(u), \text{for } j=1,2,\cdots, n
\end{equation}
where $g_j$'s are known, and $\Omega_j$ is the boundary for $f_j$ (subset where $f_j$ is known). If the underlying manifold $\mathcal{M}$ (the true rating matrix $A^*$ in the discrete setting) were known, the $n$ problems in (\ref{minenergy_all}) would be independent with each other and could be solved individually by (\ref{laplace}). However, $\mathcal{M}$ is not known, and therefore we have to get a good estimate for the operator $\Delta_{\mathcal{M}}$ based on $f_j$'s. Our algorithm for solving (\ref{minenergy_all}) is described on a high level in Algorithm \ref{alg:continuous_case}, where we iteratively update $f_j$'s and our estimate for $\Delta_{\mathcal{M}}$.

\begin{algorithm}[!t]
\caption{Algorithm for solving (\ref{minenergy_all})}
\label{alg:continuous_case} \centering
\begin{algorithmic}[1]
\REPEAT
\STATE Get estimate for $\Delta_{\mathcal{M}}$ based on $f_1,f_2,\cdots,f_n$
\FOR {$j=1$ to $n$}
\STATE Solve (\ref{laplace}) to obtain $f_j$
\ENDFOR
\UNTIL {some stopping criterion is satisfied}
\end{algorithmic}
\end{algorithm}

\textbf{Remark.} The update of $f_j$'s in Algorithm \ref{alg:continuous_case} follows the ``Jacobi'' scheme. We could also use the ``Gauss-Seidel'' scheme, i.e. re-estimate $\Delta_{\mathcal{M}}$ after the update of each $f_j$, but that would be much slower.


==> harmonic1.tex <==
Consider a user-by-item rating matrix $A=(a_{ij}) \in \mathbb{R}^{m \times n}$, where rows correspond to $m$ users, and columns correspond to $n$ items. 
The observed ratings are indexed by the set $\Omega=\{(i,j) : \text{user }i\text{ rated item }j\}$. Let $\Omega_i=\{1\le j\le m: (i,j)\in \Omega\}, \; 1\le i\le n$.
% Let our current estimate of the ratings be a matrix $R \in \mathbb{R}^{m \times n}$ (may be incomplete), and initially $R=A$.
Suppose there exists a ``true'' rating matrix $A^*$ given by an oracle with no missing entries, which is not known to us, and $A|_{\Omega} = A^*|_{\Omega}$.
%Without loss of generality, we consider the rows of $A^*$ as data points.

We formulate matrix completion as a harmonic extension problem on a manifold \cite{zgl,harmonic}. Without loss of generality, we assume that there exists a user manifold,
denoted as $\mathcal{M}$, which consists of an infinite number of users. In a user-by-item rating system, each user
is identified by an $n$-dimensional vector that consists of its ratings to $n$ items. Thus, the user manifold $\mathcal{M}$ is a submanifold embedded in $\mathbb{R}^n$.
The set of $m$ users in our user-by-item rating system is represented as $U=\{u_j, 1\le j\le m\}$ where $u_j$ is the $j$-th row of $A^*$
and $U\subset \mathcal{M}$. Let $U_i=\{u_j\in U: j\in \Omega_i\}$ be the collection of users who rate the $i$-th item. 

%For $i$-th item, we define a function $f_i: \mathcal{M}\rightarrow \mathbb{R}$ whose value is the rating to this item from different users.
For the $i$-th item, we define a function $f_i: \mathcal{M}\rightarrow \mathbb{R}$ that maps a user into the rating of this item.
From this definition, we have $f_i(u_j)=a_{ij},\; u_j\in U$ and the values of $f_i$ at $U_i$ are known. Thus the matrix completion problem is equivalent to interpolating $f_i$ from $U_i$ to $U$.

One basic observation is 
that for a fixed item, similar users should give similar ratings. This implies that the function $f_i, \; 1\le i\le n$ is a smooth function on $\mathcal{M}$. 
% Based on this observation, 
% With fixed items,
% each users is represented by a $n$-dimensional vector consisted of the rating to $n$ items. The whole user-by-item rating matrix, $A$, is equivalent to
% a point set $\mathcal{C}(A)$ in $\mathbb{R}^n$. Imaging that the number of users tends to infinity, we assume that $\mathcal{C}(A)$ becomes a submanifold embedded
% in $\mathbb{R}^n$.
% Let users be sampled from a manifold $\mathcal{M} \subset \mathbb{R}^n$, and define a real-valued function $f: \mathcal{M}^n \rightarrow \mathbb{R}$ that maps a user into the rating of some particular item. We know the function values at the points in $\partial \mathcal{M}$ (boundary condition): $f(u)|_{\partial \mathcal{M}}=g(u)$, and would like to obtain $f(u)|_{\mathcal{M} \backslash \partial \mathcal{M}}$. Thus, this can be viewed as a semi-supervised regression problem.
Therefore, it is natural to define the following energy functional:
\begin{equation}
\label{energy}
E(f) = \int_{\mathcal{M}} \|\nabla_{\mathcal{M}} f(u)\|^2 d u,
\end{equation}
where $\nabla_{\mathcal{M}} f(u)$ is the gradient at $u$ defined on the manifold $\mathcal{M}$.
Then we can interpolate $f_i$ for all the users by minimizing the energy functional in \eqref{energy}:
\begin{align}
\label{minenergy}
&\min_{f_i\in H^1(\mathcal{M})} \quad E(f_i) \quad\text{  subject to:  }\quad  f_i(u_j)|_{U_i}=a_{ij},
\end{align}
where $H^1$ is the Sobolev space.
%where $\Omega_i=\{1\le j\le m: (i,j)\in \Omega\}$.
%will encourage similar users to have similar ratings for this item. Eq. (\ref{minenergy}) is the problem we focus on.
Hence, we need to solve the following type of optimization problem for $n$ times. 
\begin{equation}
\label{opt}
\min_{f\in H^1(\mathcal{M})} \quad E(f) \quad \text{  subject to:  }\quad  f(u)|_{\Lambda}=g(u),
\end{equation}
where $\Lambda\subset\mathcal{M}$ is a point set.

To solve the above optimization problem, we first use the Bregman iteration to enforce the constraint.
\begin{itemize}
\item Solve
\begin{equation}
\label{opt-bregman} 
f^{n+1}=\arg\min_{f} \; E(f) +\mu  \|f-g+d^n\|_{L^2(\Lambda)}^2,
\end{equation}
where $\|f\|_{L^2(\Lambda)}^2=\sum_{u\in \Lambda}|f(u)|^2$, $d^n$ is a function defined on $\Lambda$.
\item Update $d^n$,
$$d^{n+1}(u)=f^{n+1}(u)-g(u),\; \forall u\in \Lambda.$$
\item Repeat above process until convergence.
\end{itemize}

\newcommand{\bx}{\mathbf{x}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bn}{\mathbf{n}}
\newcommand{\by}{\mathbf{y}}

Using a standard variational approach, the solution to (\ref{opt-bregman}) can be reduced to the following Laplace-Beltrami equation:
\begin{equation}
\label{laplace}
\begin{cases}
\displaystyle \Delta_{\mathcal{M}} f(\bx)-\mu \sum_{\by\in \Lambda} \delta(\bx-\by)(f(\by)-h(\by)) = 0, \; \bx \in \mathcal{M}, \\
\displaystyle\frac{\partial f}{\partial \mathbf{n}}(\bx)=0, \quad \bx \in \partial \mathcal{M},
\end{cases}
\end{equation}
where $\delta$ is the Dirac-$\delta$ function in $\mathcal{M}$, $h=g-d^n$ is a given function on $\Lambda$, and $\mathbf{n}$ is the outer normal vector.
That is to say, the function $f$ that minimizes (\ref{opt}) is a harmonic function on $\mathcal{M} \backslash \partial \mathcal{M}$, and (\ref{laplace}) is called the {\em harmonic extension} problem in the continuous setting.

% Now we will extend the above theory to predict the ratings for all the items in a data set. Let us use $f_1,f_2,\cdots,f_n: \mathcal{M} \rightarrow \mathbb{R}$ to denote the functions that map a user to the ratings of item $1$, item $2$, $\cdots$, item $n$, respectively.

% We consider the energy minimization problems
% \begin{equation}
% \label{minenergy_all}
% \min_{f_j} E(f_j) \text{  subject to  } f_j(u)|_{\Omega_j}=g_j(u), \text{for } j=1,2,\cdots, n
% \end{equation}
% where $g_j$'s are known, and $\Omega_j$ is the boundary for $f_j$ (subset where $f_j$ is known).

If the underlying manifold $\mathcal{M}$ (the true rating matrix $A^*$ in the discrete setting) were known, the $n$ problems in (\ref{minenergy}) would be independent with each other and could be solved individually by (\ref{laplace}). However, $\mathcal{M}$ is not known, and therefore we have to get a good estimate for the operator $\Delta_{\mathcal{M}}$ based on $f_j$'s. Our algorithm for solving (\ref{minenergy}) is described on a high level in Algorithm \ref{alg:continuous_case}, where we iteratively update $f_j$'s and our estimate for $\Delta_{\mathcal{M}}$.

In the next section, we use the point integral method (PIM) to solve the Laplace-Beltrami equation \eqref{laplace}.

\begin{algorithm}[!t]
\caption{Algorithm for solving (\ref{minenergy})}
\label{alg:continuous_case} \centering
\begin{algorithmic}[1]
\REPEAT
\STATE Get estimate for $\Delta_{\mathcal{M}}$ based on $f_1,f_2,\cdots,f_n$
\FOR {$i=1$ to $n$}
\STATE Solve (\ref{laplace}) to obtain $f_i$
\ENDFOR
\UNTIL {some stopping criterion is satisfied}
\end{algorithmic}
\end{algorithm}

\textbf{Remark.} The update of $f_j$'s in Algorithm \ref{alg:continuous_case} follows the ``Jacobi'' scheme. We could also use the ``Gauss-Seidel'' scheme, i.e. re-estimate $\Delta_{\mathcal{M}}$ after the update of each $f_j$, but that would be much slower.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper0104"
%%% End:


==> intro0.tex <==
Recommender systems are crucial components in contemporary e-commerce platforms (Amazon, eBay, Netflix, etc.), and were popularized by the Netflix challenge. As the volume of users and items becomes increasingly larger, the computational efficiency and quality of recommendation are equally important in practical use. Detailed surveys of this field can be found in [][]. This paper addresses both the efficiency and quality aspects of recommender systems.

Recommendation algorithms are commonly based on collaborative filtering, or ``crowd of wisdom'', and can be categorized into memory-based and model-based approaches. Memory-based approaches include user-based and item-based recommendation. For example, for a user $u$, we retrieve the highly-rated items from the nearest neighbors of $u$, and recommend those items that have not been consumed by $u$. Memory-based methods are actually based on a graph, where a user-user or item-item similarity matrix defines the nearest neighbors of each user or item. In contrast, model-based methods are formulated as matrix completion problems which assume that the entire user-by-item rating matrix is low-rank, and the goal is to predict the missing ratings given the observed ratings. While memory-based methods are typically more computationally efficient, model-based methods can achieve much higher quality for collaborative filtering.

Popular model-based methods such as regularized SVD minimize the sum-of-squares error over all the observed ratings. When evaluating the predictive accuracy of these algorithms, we often divide the whole data set into a training set and a test set. After obtaining a model on the training set, we evaluate the accuracy of the model's prediction on the test set in order to see how well it generalizes to unseen data. However, the measure for evaluating success in a practical recommender system is very different. What we care more about is whether the top recommended items for a user $u$ will actually be ``liked'' by $u$. In an experimental setting, the evaluation measure for success in this context is the resemblance between the ranked list of top recommended items and the ranked list of observed ratings in the test set. Thus, this measure that compares two rankings is more relevant to the performance in real scenarios. The problem that places priority on the top recommended items rather than the absolute accuracy of predicted ratings is referred to as top-N recommendation, or more recently {\em collaborative ranking}, and is our focus in this paper.

When considering the computational efficiency of a recommendation algorithm, we would need to take both the training phase and testing phase into account. In the testing phase, when the outcome of the algorithm is a ranked list of items for some user, as in the collaborative ranking setting, regularized SVD and other matrix factorization methods have to compute the ratings for all the items and return the top-rated ones to the user, which is only a small subset of all the items. On the contrary, what we would prefer is an algorithm that outputs the ranked list of top recommended items directly, like the memory-based approaches, and consequently, we can save the computation time that would otherwise be wasted for computing the ratings for the items not returned to the user eventually.

In this paper, we propose a fast graph-based method for collaborative ranking. Our method differs from existing approaches in two important ways: \newline (1) We start with the same matrix completion problem as in model-based methods, but formulate it as a series of semi-supervised learning problems, or in particular, harmonic extension problems that can be solved by label propagation. For each item, we want to know the ratings by all the users, and the goal of the semi-supervised learning problem is to propagate the known labels for this item (observed ratings) to the unknown labels on the user-user graph; and reversely, for each user, to propagate the known labels given by this user to the unknown labels on the item-item graph. Inherently, our method does not impose a low-dimensional Euclidean subspace structure; as shown in the supplementary material, our method can be viewed as minimizing the dimension of the user or item manifold. \newline (2) For better scalability, we don't intend to fill in all the missing ratings. Instead, for each item, we consider only the users who are most likely to rate this item; or reversely, for each user, we consider only the items that are most likely to be rated by this user. Therefore, we are trying to partially solve the harmonic extension problems by {\em local} propagation of the labels, and we expect the partial solutions to be useful for the sake of collaborative ranking.

An important aspect of our proposed method is the similarity matrix that defines the user-user or item-item graph. Because the information given in the rating matrix is incomplete, we can only assume that the similarity matrix used in harmonic extension is a good guess. We will illustrate that the typical cosine similarity matrix used in traditional memory-based methods has inherent drawbacks, and propose a new way to construct the similarity matrix based on incomplete data.

Our contribution is summarized as follows:
\begin{itemize}
\item We propose an efficient algorithm that exploits local graph structures to solve the harmonic extension problem for collaborative ranking.
\item We present a new way to form the user or item similarity matrix with incomplete data and iteratively improve it, which is useful for other graph-based methods for recommendation.
\item Overall, our proposed approach achieves high-quality ranking results in considerably less time compared to state-of-the-art methods. The experiments on the Yahoo! Music data set with 700 million nonzeros demonstrate the usefulness of our approach for industry-level recommender systems.
\end{itemize}

The rest of this paper is organized as follows. In Section \ref{harmonic}, we formulate the matrix completion problem as harmonic extension. In Section \ref{discretization}, we describe the point integral method (PIM) to rigorously solve the discretized harmonic extension. In Section \ref{LPIM}, we partially solve the harmonic extension problem using an efficient localized PIM for generating top recommended items. In Section \ref{sim_matrix}, we describe our efficient and more rigorous way to compute the similarity matrix. In Section \ref{experiments}, we empirically demonstrate the efficiency and quality of our method. In Section \ref{related}, we explain the connection and difference between our method and previous work. In Section \ref{conclusion}, we discuss our proposed method and its implication on other methods.

Here are some notations we will use. For a vector $x=[x_1,\cdots,x_m]^T$, we call $y=[x_{i_1},x_{i_2},\cdots,x_{i_r}]^T$ a {\em subvector} of length $r$ by extracting the elements of $x$ in the index set $\{i_1,\cdots,i_r\}$, where $i_1<i_2<\cdots<i_r$. For a matrix $M$, a vector $x$, integers $i,j$, and sets of row and column indices $S,S'$, we use $M_{i,j},M_{S,S'},M_{:,j},M_{S,j},x_S$ to denote an entry of $M$, a submatrix of $M$, the $j$-th column of $M$, a subvector of the $j$-th column of $M$, and a subvector of $x$, respectively.


==> intro1.tex <==
Recommender systems are crucial components in contemporary e-commerce platforms (Amazon, eBay, Netflix, etc.), and were popularized by the Netflix challenge \cite{netflix}.
%As the volume of users and items becomes increasingly larger, the computational efficiency and quality of recommendation are equally important in practical use.
Detailed surveys of this field can be found in \cite{rssurvey1, rssurvey2}.
%This paper addresses both the efficiency and quality aspects of recommender systems.
Recommendation algorithms are commonly based on collaborative filtering, or ``crowd of wisdom'', and can be categorized into memory-based and model-based approaches. Memory-based approaches include user-based and item-based recommendation \cite{itembased}. For example, for a user $u$, we retrieve the highly-rated items from the nearest neighbors of $u$, and recommend those items that have not been consumed by $u$. Memory-based methods are actually based on a graph, where a user-user or item-item similarity matrix defines the nearest neighbors of each user or item. In contrast, model-based methods are formulated as matrix completion problems which assume that the entire user-by-item rating matrix is low-rank \cite{svdcf}, and the goal is to predict the missing ratings given the observed ratings. While memory-based methods are typically more computationally efficient, model-based methods can achieve much higher quality for collaborative filtering.

Popular model-based methods such as regularized SVD \cite{svdcf} minimize the sum-of-squares error over all the observed ratings. When evaluating the predictive accuracy of these algorithms, we often divide the whole data set into a training set and a test set. After obtaining a model on the training set, we evaluate the accuracy of the model's prediction on the test set in order to see how well it generalizes to unseen data. However, the measure for evaluating success in a practical recommender system is very different. What we care more about is whether the top recommended items for a user $u$ will actually be ``liked'' by $u$. In an experimental setting, the evaluation measure for success in this context is the resemblance between the ranked list of top recommended items and the ranked list of observed ratings in the test set. Thus, this measure that compares two rankings is more relevant to the performance in real scenarios. The problem that places priority on the top recommended items rather than the absolute accuracy of predicted ratings is referred to as top-N recommendation \cite{eval_topn2}, or more recently {\em collaborative ranking} \cite{lcr, altsvm}, and is our focus in this paper.

%When considering the computational efficiency of a recommendation algorithm, we would need to take both the training phase and testing phase into account. In the testing phase, when the outcome of the algorithm is a ranked list of items for some user, as in the collaborative ranking setting, regularized SVD and other matrix factorization methods have to compute the ratings for all the items and return the top-rated ones to the user, which is only a small subset of all the items. On the contrary, what we would prefer is an algorithm that outputs the ranked list of top recommended items directly, like the memory-based approaches, and consequently, we can save the computation time that would otherwise be wasted for computing the ratings for the items not returned to the user eventually.

%In this paper, we propose a fast graph-based method for collaborative ranking. Our method differs from existing approaches in two important ways: \newline (1)
In this paper, we propose a graph-based method for collaborative ranking. Built upon the same user-user or item-item graph in memory-based collaborative filtering, our method rigorously learns the underlying user or item manifold.
We start with the same matrix completion problem as in model-based methods, but formulate it as a series of semi-supervised learning problems, or in particular, harmonic extension problems that can be solved by label propagation. For each item, we want to know the ratings by all the users, and the goal of the semi-supervised learning problem is to propagate the known labels for this item (observed ratings) to the unknown labels on the user-user graph; and reversely, for each user, to propagate the known labels given by this user to the unknown labels on the item-item graph. The harmonic extension problems are defined in a continuous domain (the user or item manifold), which results in partial differential equations (PDEs) each involving the Laplace-Beltrami operator with a Dirichlet boundary \cite{neumann}. We solve the PDEs numerically using an advanced point integral method (PIM) \cite{harmonic}. Inherently, we will show that our method does not impose a low-dimensional Euclidean subspace structure, but can be viewed as minimizing the dimension of the user or item manifold. 
%\newline (2) For better scalability, we don't intend to fill in all the missing ratings. Instead, for each item, we consider only the users who are most likely to rate this item; or reversely, for each user, we consider only the items that are most likely to be rated by this user. Therefore, we are trying to partially solve the harmonic extension problems by {\em local} propagation of the labels, and we expect the partial solutions to be useful for the sake of collaborative ranking.

An important aspect of our proposed method is the weight matrix that defines the user-user or item-item graph. Because the information given in the rating matrix is incomplete, we can only assume that the weight matrix used in harmonic extension is a good guess. We will propose an efficient way to construct the weight matrix based on incomplete data.

Our contribution is summarized as follows:
\begin{itemize}
\item We propose an algorithm that exploits manifold structures to solve the harmonic extension problem for collaborative ranking, representing a new perspective on graph-based methods for recommender systems.
\item On real data sets, our method achieves robust ranking quality with reasonable run-time, compared to state-of-the-art methods for large-scale recommender systems.
\end{itemize}

The rest of this paper is organized as follows. In Section \ref{harmonic}, we formulate the matrix completion problem as harmonic extension. In Section \ref{discretization}, we describe the point integral method (PIM) to rigorously solve the discretized harmonic extension problem. In Section \ref{LDMM}, we show that our approach seeks to minimize the dimension of the underlying manifold. In Section \ref{pairwiseranking}, we connect our formulation with pairwise ranking loss minimization. In Section \ref{sim_matrix}, we describe our efficient and more rigorous way to compute the similarity matrix. In Section \ref{experiments}, we empirically demonstrate the efficiency and quality of our method. In Section \ref{related}, we explain the connection and difference between our method and previous work. In Section \ref{conclusion}, we discuss our proposed method and its implication on other methods.

Here are some notations we will use. For a vector $x=[x_1,\cdots,x_m]^T$, we call $y=[x_{i_1},x_{i_2},\cdots,x_{i_r}]^T$ a {\em subvector} of length $r$ by extracting the elements of $x$ in the index set $\{i_1,\cdots,i_r\}$, where $i_1<i_2<\cdots<i_r$. For a matrix $M$, a vector $x$, integers $i,j$, and sets of row and column indices $S,S'$, we use $M_{i,j},M_{S,S'},M_{:,j},M_{S,j},x_S$ to denote an entry of $M$, a submatrix of $M$, the $j$-th column of $M$, a subvector of the $j$-th column of $M$, and a subvector of $x$, respectively.


==> pairwise.tex <==
We notice that 

